A stable FSI algorithm for light rigid bodies in compressible flow

In this article we describe a stable partitioned algorithm that overcomes the added mass instability arising in fluid-structure interactions of light rigid bodies and inviscid compressible flow. The new algorithm is stable even for bodies with zero mass and zero moments of inertia. The approach is based on a local characteristic projection of the force on the rigid body and is a natural extension of the recently developed algorithm for coupling compressible flow and deformable bodies. Normal mode analysis is used to prove the stability of the approximation for a one-dimensional model problem and numerical computations confirm these results. In multiple space dimensions the approach naturally reveals the form of the added mass tensors in the equations governing the motion of the rigid body. These tensors, which depend on certain surface integrals of the fluid impedance, couple the translational and angular velocities of the body. Numerical results in two space dimensions, based on the use of moving overlapping grids and adaptive mesh refinement, demonstrate the behavior and efficacy of the new scheme. These results include the simulation of the difficult problem of a shock impacting an ellipse of zero mass.

==> texFiles/model.tex <==
\section{A model problem for compressible gas/solid body coupling} \label{sec:model}
Consider a 1-D model problem of a rigid body confined on either side by an inviscid compressible fluid. As in~\cite{banks11a} we can linearize and freeze coefficients about a reference state to arrive at a problem where the equations of linear elasticity govern the two fluids and Newtonian mechanics govern the motion of the solid. This situation is displayed pictorially in figure~\ref{fig:modelFig}
%
\input{texFiles/modelFig.tex}
%
More specifically, for the left fluid
%
\begin{equation}
  \left[\begin{array}{c}
    \uL\\
    \sigmaL
  \end{array}\right]_t-
  \left[\begin{array}{cc}
    0 \quad& \frac{1}{\rhoL} \\
    \kappaL \quad& 0
  \end{array}\right]
  \left[\begin{array}{c}
    \uL\\
    \sigmaL
  \end{array}\right]_x=0,
  \quad\hbox{for} \quad x < -\frac{L}{2},
  \label{eq:LELeft}
\end{equation}
%
for the right fluid
\begin{equation}
  \left[\begin{array}{c}
    \uR\\
    \sigmaR
  \end{array}\right]_t-
  \left[\begin{array}{cc}
    0 \quad& \frac{1}{\rhoR} \\
    \kappaR \quad& 0
  \end{array}\right]
  \left[\begin{array}{c}
    \uR\\
    \sigmaR
  \end{array}\right]_x=0,
  \quad\hbox{for} \quad x > \frac{L}{2},
  \label{eq:LERight}
\end{equation}
%
and for the rigid body
\begin{equation}
 \left[\begin{array}{c}
    \vRB
 \end{array}\right]_t = \frac{\force}{\mass}%\frac{\sigmaR(\frac{L}{2},t)-\sigmaL(-\frac{L}{2},t)}{\mass}.
 \label{eq:RBMotion}
\end{equation}
%
where 
\begin{equation}
  \force =\left.\sigmaR\right|_{x=\frac{L}{2}}-\left.\sigmaL\right|_{x=-\frac{L}{2}}.\label{eq:ic1}
\end{equation}
%
The system is closed using interface conditions at $x=\pm L/2$ which enforce continuity of velocity, namely
%
\begin{align}
  \left.\uL \right|_{x=-\frac{L}{2}} & = \vRB \label{eq:ic2}\\
  \left.\uR \right|_{x=\frac{L}{2}} & = \vRB.\label{eq:ic3}
\end{align}
%
Notice that the problem is posed in the reference frame (which we call here $x$), but the deformed state attached to the rigid body can be calculated as
\begin{equation}
    \hat{x} = x+\int_0^t \vRB \, dt.
\end{equation}


==> texFiles/modelSpaceTime.tex <==
%
% Cartoon showing the displaced frame
%
\begin{figure}[hbt]
\begin{center}
\begin{tikzpicture}[scale=3]
%
% axes: 
\draw[->] (-1.,0) -- (1.,0) node[anchor=south] {$\hat{x}$};
\draw[->] (0,0) -- (0,1) node[anchor=west] {$t$} ;
%
% - piston:
\draw[very thick,green] (0,0) .. controls (-.5,.5) and (-.1,0.7) .. (-.1,.8); 
\draw[very thick,green] (.5,0) .. controls (0,.5) and (.4,.7) .. (.4,.8); 

%node[anchor=south,yshift=-2pt,blue] {$x=U(t)$};
%\draw[very thick,green](0,0)
\draw[black] (-.4,.8) node[anchor=south,yshift=10pt,xshift=-7pt] {$a=0$};
%
\end{tikzpicture}
\end{center}
\caption{An $x-t$ diagram for the test setup of figure~\ref{fig:modelFig}. At left is the diagram in the reference coordinate $x$ while at right is the diagram in the displaced coordinate system $\hat{x}=x+U(x,t)$.} \label{fig:modelSpaceTime}
\end{figure}

==> texFiles/motivation.tex <==
\section{Motivation} \label{sec:motivation}
\subsection{Numerical approximations}\label{sec:simpleInterior}
 
This section describes the discretization of (\ref{eq:LELeft}) and (\ref{eq:LERight}).
%We are interested in computational simulation and so now present a basic numerical setup 
%for the proposed test problem.
As in~\cite{banks11a}, Godunov style upwind discretizations will be used for the fluid domains
to demonstrate and analyze the features of various discrete interface conditions. 

The finite difference grid for the discretization of the one dimensional 
problem is outlined in Fig.~\ref{fig:oneddisc}.
\begin{figure}
\begin{center}
\includegraphics[width=0.60\textwidth]{images/domain}
\end{center}
\caption{Finite difference grid.}
\label{fig:oneddisc}
\end{figure}
The grid points to the left of the rigid body are denoted by
%
\begin{equation}
  x_{L,i} = -\frac{L}{2}+\left(i+\frac{1}{2}\right)\dxL,\quad i=\ldots, -2,-1,0,
\end{equation}
%
and to the right by 
%
\begin{equation}
  x_{R,i} = \frac{L}{2}+\left(i-\frac{1}{2}\right)\dxR,\quad i=0,1,2,\ldots .
\end{equation}
%
The ghost points, $i=0$ for both domains, will be used to enforce interface conditions. 

The eigendecomposition of the matrices in (\ref{eq:LELeft}) and (\ref{eq:LERight}) are given by 
\begin{equation}
  \left[\begin{array}{cc}
    0 & \frac{1}{\rho_k}\medskip\\
  \kappa_k & 0
  \end{array}\right]=
  %
  R_k\Lambda_k R^{-1}_k = 
  \left[\begin{array}{cc}
    -c_k & c_k \medskip \\
    \kappa_k & \kappa_k
  \end{array}\right]
  %
  \left[\begin{array}{cc}
    -c_k & 0\medskip\\
   0 & c_k
  \end{array}\right]
  %
  \left[\begin{array}{cc}
      -\frac{1}{2 c_k} & \frac{1}{2 \kappa_k}\medskip\\
      \frac{1}{2 c_k} & \frac{1}{2 \kappa_k}
  \end{array}\right]
\end{equation}
where the wave speed is $c_k=\sqrt{\kappa_k/\rho_k}$ and $k=L$ or $R$. 
The first order upwind method for each domain $k=L,R$ is compactly written
%
\begin{equation}
    \uLE{k}_i^{n+1} =  
    \uLE{k}_i^{n} 
    %
    +\Delta t R_k\Lambda_k^{-}R_k^{-1}
    \Dp \uLE{k}_i^n
    %
    +\Delta tR_k\Lambda_k^{+}R_k^{-1}
      \Dm \uLE{k}_i^n
  \label{eq:discreteInterior_fo}
\end{equation}
for $i=\ldots,-2,-1$ to the left and for $i=1,2\ldots$ to the right.
The negative and positive parts of the wave speeds are defined by
\begin{equation}
  \Lambda_k^{-} = 
  \left[\begin{array}{cc}
    -c_k & 0\\
   0 & 0
  \end{array}\right] \quad\hbox{and}\quad
  %
  \Lambda_k^{+} = 
  \left[\begin{array}{cc}
    0 & 0\\
   0 & c_k
  \end{array}\right]
\end{equation}
respectively. The forward and backward divided differences are defined by $D_+u_i=(u_{i+1}-u_i)/\Delta x$ and 
$D_-u_i = D_+u_{i-1}$.

The backward Euler update,
%
\begin{equation}
  \vRB^{n+1} = \vRB^n+\frac{\Delta t}{\mass} \force^{n+1},
  \label{eq:BE}
\end{equation}
%
approximates the equation for the solid (\ref{eq:RBMotion}). The force at $t_{n+1}$, $F^{n+1}$, will be defined by a
discretization of the interface condition (\ref{eq:ic1}). 
The backward Euler method is used here in order to simplify the discussion. We will be addressing the question 
of the stability of the coupling, not the rigid body integrator itself. An unconditionally 
stable ODE integrator, such as backward Euler, will not give any constraint on the stable time step by itself.
Therefore, any time step constraint in addition to the CFL condition in the fluid domains that results from the analysis
below, will be due to the coupling procedure.
Moreover, since (\ref{eq:RBMotion}) is a scalar ODE, the computational cost of an implicit time 
integrator is very low. However, the use of implicit methods in not essential and one 
could consider an explicit approach with sub-cycling, for example. Some discussion of these issues will be provided 
where appropriate.
\par
In summary, the numerical schemes (\ref{eq:discreteInterior_fo}) and (\ref{eq:BE}) approximate the 
equations (\ref{eq:LELeft}), (\ref{eq:LERight}), and (\ref{eq:RBMotion}) to
first order accuracy.  The discrete scheme for the full system will be completely described by imposing 
a numerical approximation of the interface conditions (\ref{eq:ic1}), (\ref{eq:ic2}), and (\ref{eq:ic3}). 
These interface conditions will 
define the force applied to the body and the boundary conditions for the two fluids. In the following sections,
it will be shown that different ways of imposing (\ref{eq:ic1})--(\ref{eq:ic3}) will lead to very different behaviors
of the coupled approximation.

%%%%%%%%%%%%%
\subsection{Traditional coupling technique}\label{sec:traditionalc}
In the literature, the standard enforcement of the interface conditions can be described as applying the 
velocity from the solid as a boundary condition on the fluids, and applying the stress in the fluid to derive 
the applied force on the body. A straightforward first order implementation is as follows. 
Assume that the solution is given at time $t_n$, That is, assume $\uLE{L}_i^n$ for $i=\ldots,-1,0$, $\uLE{R}_i^n$ for
$i=0,1,\dots$, and $\vRB^n$ are known. To advance one time step
\begin{enumerate}
\item Compute $\uLE{L}_i^{n+1}$ for $i=\ldots,-2,-1$ and $\uLE{R}_i^{n+1}$ for $i=1,2,\ldots$ by 
(\ref{eq:discreteInterior_fo}).
\item Set $F^{n+1} = \sigma_{R,1}^{n+1}-\sigma_{L,-1}^{n+1}$, and compute $\vRB^{n+1}$ by (\ref{eq:BE}).
\item Define the ghost point values by the velocity boundary condition
\begin{align}
  \uL_{0}^{n+1} = \vRB^{n+1} \\
  \uR_{0}^{n+1} = \vRB^{n+1}
\end{align}
and the stress extrapolation
\begin{align}
  \sigmaL_{0}^{n+1} = \sigmaL_{-1}^{n+1} \label{eq:icn1}\\
  \sigmaR_{0}^{n+1} = \sigmaR_{1}^{n+1}.\label{eq:icn2}
\end{align}
\end{enumerate}
This discrete condition works well in many cases, but for problems where the solid is sufficiently light compared 
to the fluids a known instability occurs (reference???). 
One common approach to eliminating this instability is to move to a fully implicit monolithic approach where the various 
sub-domains are considered as one large system rather than a partitioned approach such as we have described.
We will analyze this instability below, and show that it is possible to modify the interface conditions 
(\ref{eq:icn1}) and (\ref{eq:icn2}) to avoid this unstable behavior.

%%%%%%%%%%%%%
\subsection{Derivation of a new coupling technique}\label{sec:newc}
%\subsection{A thought experiment and a new coupling technique}
In order to derive a new numerical approach to coupling, we pursue a thought experiment. Instead of the rigid solid in Figure~\ref{fig:modelFig}, consider that the solid is compressible and its motions are governed by the equations of linearly elasticity with density $\rho_S=\mass/L$ and $\kappa=\kappa_{RB}$. Here $\kappa_{RB}$ will be taken as a parameter and we will investigate what happens as it is allowed to trend to $\infty$. Unknown velocity ($v_{RB}$) and stress ($\sigma_{RB}$), which are functions of space and time, are introduced in this new solid body. The discussion in~\cite{banks11a} is directly applicable to this modified case and so we define velocities and stresses at $x=\pm L/2$ using the techniques discussed in that work. It was found in~\cite{banks11a} that impedance weighting of the the interfacial velocity and stress was a useful concept and could lead to numerical methods with favorable stability constraints. In the current context this weighting is written
%
\begin{align}
  \sigma_{I,L} & = \frac{1}{z_L+z_{RB}}\left(z_{RB}\left.\sigmaL\right|_{x=-\frac{L}{2}}+z_{L}\left.\sigma_{RB}\right|_{x=-\frac{L}{2}}+z_{L}z_{RB}\left(\left.v_{RB}\right|_{x=-\frac{L}{2}}-\left.\uL\right|_{x=-\frac{L}{2}}\right)\right) \\
  %
  \sigma_{I,R} & = \frac{1}{z_{RB}+z_{R}}\left(z_{R}\left.\sigma_{RB}\right|_{x=\frac{L}{2}}+z_{RB}\left.\sigmaR\right|_{x=\frac{L}{2}}+z_{R}z_{RB}\left(\left.\uR\right|_{x=\frac{L}{2}}-\left.v_{RB}\right|_{x=\frac{L}{2}}\right)\right) \\
  %
  v_{I,L} & = \frac{1}{z_L+z_{RB}}\left(z_{L}\left.\uL\right|_{x=-\frac{L}{2}}+z_{RB}\left.v_{RB}\right|_{x=-\frac{L}{2}}+\left.\sigma_{RB}\right|_{x=-\frac{L}{2}}-\left.\sigmaL\right|_{x=-\frac{L}{2}}\right) \\
  %
  v_{I,R} & = \frac{1}{z_{RB}+z_{R}}\left(z_{RB}\left.v_{RB}\right|_{x=\frac{L}{2}}+z_{R}\left.\uR\right|_{x=\frac{L}{2}}+\left.\sigmaR\right|_{x=\frac{L}{2}}-\left.\sigma_{RB}\right|_{x=\frac{L}{2}}\right)
\end{align}
%
where $z_L=\rhoL\kappaL$, $z_{RB}=\rho_{RB}\kappa_{RB}$, and $z_R=\rhoR\kappaR$. Here $\sigma_{I,k}$ and $v_{I,k}$ are the interfacial stress and velocity at the boundary between fluid and solid domains. Now we take the limit $\kappa_{RB}\to\infty$ which gives $z_{RB}\to \infty$, from whence
%
\begin{align}
  \sigma_{I,L} & = \left.\sigmaL\right|_{x=-\frac{L}{2}}+{z_{L}}\left(\left.v_{RB}\right|_{x=-\frac{L}{2}}-\left.\uL\right|_{x=-\frac{L}{2}}\right) \\
  %
  \sigma_{I,R} & = \left.\sigmaR\right|_{x=\frac{L}{2}}+{z_{R}}\left(\left.\uR\right|_{x=\frac{L}{2}}-\left.v_{RB}\right|_{x=\frac{L}{2}}\right) \\
  %
  v_{I,L} & = \left.v_{RB}\right|_{x=-\frac{L}{2}} \\
  %
  v_{I,R} & = \left.v_{RB}\right|_{x=\frac{L}{2}}.
\end{align}
%
Notice that the stress within the body becomes irrelevant (it need not be maintained as a dependent variable), and because the body becomes rigid as $\kappa_{RB}\to\infty$, the velocity throughout the solid can be replaced by the velocity of the center of mass. Thus the limiting behavior of the impedance weighted boundary conditions  for $\kappa_{RB}\to\infty$ is
%
\begin{align}
  \sigma_{I,L} & = \left.\sigmaL\right|_{x=-\frac{L}{2}}+{z_{L}}\left(\vRB-\left.\uL\right|_{x=-\frac{L}{2}}\right) \\
  %
  \sigma_{I,R} & = \left.\sigmaR\right|_{x=\frac{L}{2}}+{z_{R}}\left(\left.\uR\right|_{x=\frac{L}{2}}-\vRB\right) \\
  %
  v_{I,L} & = \vRB \\
  %
  v_{I,R} & = \vRB.
\end{align}

This new coupling condition can be implemented in the context of the simple numerical methods in Section~\ref{sec:simpleInterior} as follows. Define the interface stresses at $t_n$ using first order extrapolation and projection as
%
\begin{align}
  \sigma_{I,L}^n & = \sigmaL_0^n+{z_{L}}\left(\vRB^n-\uL_0^n\right) \\
  %
  \sigma_{I,R}^n & = \sigmaR_0^n+{z_{R}}\left(\uR_0^n-\vRB^n\right).
\end{align}
%
Assume $\uLE{k}_i^n$ for $k=L,R$ and $i=0,1,\ldots$, and $\vRB^n$ are known. The velocity from the solid can be applied as a boundary condition on the fluids by setting
\begin{align}
  \uL_{-1}^n = \vRB^n \label{eq:vLeftFO}\\
  \uR_{-1}^n = \vRB^n \label{eq:vRightFO}.
\end{align}
Extrapolation of the stress to the ghost cells gives
\begin{align}
  \sigmaL_{-1}^n = \sigma_{I,L}^n \label{eq:stressLeftFO}\\
  \sigmaR_{-1}^n = \sigma_{I,R}^n \label{eq:stressRightFO}.
\end{align}
Equation (\ref{eq:discreteInterior_fo}) is then used to update fluid quantities for both domains for $i=0,1,\ldots$. The force is defined from the fluid domains as 
\begin{equation}
  \force^{n+1} = \sigma_{I,R}^n-\sigma_{I,L}^n = \sigmaR_0^{n+1}+{z_R}\left(\uR_0^{n+1}-\vRB^{n+1}\right)-\sigmaL_0^{n+1}-{z_L}\left(\vRB^{n+1}-\uL_0^{n+1}\right)\label{eq:icnew}
\end{equation}
and (\ref{eq:BE}) is used to advance the solid variables by solving a simple implicit equation for the scalar unknown $\vRB^{n+1}$. Note that instead of the backward Euler integration for the rigid body, one could use an explicit integrator with an appropriate number of sub-cycles. The numerical implementation is straightforward, but notational difficulties make a full analysis somewhat cumbersome.

\subsection{Normal mode analysis}\label{sec:normalMode}
To summarize, a general coupling technique with weights $\alpha_L$ and $\alpha_R$ is written as
the stress extrapolation and velocity continuity
\begin{alignat}{2}
 \sigmaL_{0}^{n} = \sigma_{I,L}^n \qquad &\sigmaR_{0}^n = \sigma_{I,R}^n \\
 \uL_0^n = \vRB^n \qquad & \uR_0^n = \vRB^n,
\end{alignat}
and the rigid body force
$$
 F^{n} = \sigma_{I,R}^n - \sigma_{I,L}^n,
$$
with interface stresses
\begin{align}
  \sigma_{I,L}^n  = \sigmaL_{-1}^n+{\alpha_{L}}\left(\vRB^n-\uL_{-1}^n\right)  \label{eq:genStressLeft} \\
  %
  \sigma_{I,R}^n  = \sigmaR_1^n+{\alpha_{R}}\left(\uR_1^n-\vRB^n\right), \label{eq:genStressRight}
\end{align}
The traditional coupling technique in Sec.~\ref{sec:traditionalc} is obtained for $\alpha_L=\alpha_R=0$ and the 
new coupling technique of Sec.~\ref{sec:newc} is obtained for $\alpha_L=\rho_Lc_L$, $\alpha_R=\rho_Rc_R$.
To enforce these conditions, assume that the solution is given at time $t_n$, and perform the 
following substeps to advance to time $t_{n+1}$.
\begin{enumerate}
\item Compute $\uLE{L}_i^{n+1}$ for $i=\ldots,-2,-1$ and $\uLE{R}_i^{n+1}$ for $i=1,2,\ldots$ by 
(\ref{eq:discreteInterior_fo}).
\item Set $F^{n+1} = \sigma_{R,1}^{n+1}+\alpha_R(\uR^{n+1}_1-\vRB^{n+1}) - 
      \sigma_{L,-1}^{n+1} - \alpha_L(\vRB^{n+1}-\uL^{n+1}_{-1})$, and 
     solve (\ref{eq:BE}) for $\vRB^{n+1}$, 
\begin{equation}
\left(1+\frac{\Delta t}{M}(\alpha_L+\alpha_R)\right)\vRB^{n+1} = \vRB^n + 
   \frac{\Delta t}{M}\left(  \sigma^{n+1}_{R,1} +\alpha_R\uR^{n+1}_1 - 
                            (\sigma^{n+1}_{L,-1}+\alpha_L\uL^{n+1}_{-1})\right)
\label{eq:eqforv}
\end{equation}
\item Define the ghost point values by the velocity boundary condition
\begin{align}
  \uL_{0}^{n+1} = \vRB^{n+1} \\
  \uR_{0}^{n+1} = \vRB^{n+1}
\end{align}
and the stress extrapolation
\begin{align}
  \sigmaL_{0}^{n+1} = \sigmaL_{-1}^{n+1} + \alpha_L(\vRB^{n+1}-\uL_{-1}^{n+1}) \\
  \sigmaR_{0}^{n+1} = \sigmaR_{1}^{n+1}  + \alpha_R(\uR_1^{n+1}-\vRB^{n+1}).
\end{align}
\end{enumerate}
Next, we analyze the stability of these conditions, and investigate how the choice of $\alpha$ affects the
behavior of the overall numerical method.
\par
To simplify the presentation, assume $\kappaL=\kappaR=\kappa$, $\rhoL=\rhoR=\rho$, $\dxL=\dxR=\dx$, and
$\alpha_L=\alpha_R=\alpha$.
This assumption is purely for convenience and clarity, and does not materially change the results of 
the analysis. We pursue a stability analysis via the normal mode theory of Gustafsson Kreiss and 
Sundstr{\"o}m (GKS)~\cite{gustafsson72}. 
%The discussion is simplified somewhat by introducing a unifying notation 
%for the stress at the left and right of the solid as 
%
%
%\begin{align}
%  \sigma_{I,L}^n & = \sigmaL_0^n+{\alpha}\left(\vRB^n-\uL_0^n\right)\\
%  %
%  \sigma_{I,R}^n & = \sigmaR_0^n+{\alpha}\left(\uR_0^n-\vRB^n\right)
%\end{align}
%
%where $\alpha$ is a projection weight to be determined. 
As was done in~\cite{banks11a}, normal mode solutions of the form
\begin{equation}
  \uLE{k}_i^n = A^n
  %
  \left[\begin{array}{c}
    \tilde{v}_k\\
    \tilde{\sigma}_k
  \end{array}\right]_i, \qquad
  \vRB^n = A^n \tilde{\vRB}\qquad k=L,R\label{eq:normalmode}
\end{equation}
where $\tilde{v}_{k,i}$ and $\tilde{\sigma}_{k,i}$ are bounded functions of space, and $A$ is a complex scalar
with $|A|>1$, are sought. If such a solution can be found, the approximation grows unboundedly in time.
%As shown in \cite{gustafsson72}, also the oposite is true, i.e., that if no soultions of the 
%form (\ref{eq:normalmode}) with $|A|>1$, or with $|A|=1$ such that $|A| \rightarrow 1+$ exist, then 
%the solution is stable. 

Characteristic normal modes are denoted by
\begin{equation}
  \left[\begin{array}{c}
    a_k\\
    b_k
  \end{array}\right] = R_k^{-1}
  \left[\begin{array}{c}
    \tilde{u}_k\\
    \tilde{\sigma}_k
  \end{array}\right].
  \label{eq:char_normal_modes}
\end{equation}
%
Insertion of (\ref{eq:normalmode}) into the finite difference scheme (\ref{eq:discreteInterior_fo}) leads
to difference equations for $[\tilde{u}_k\ \tilde{\sigma}_k]$. The solutions of these difference equations
together with the assumption of boundedness as $i\rightarrow \pm\infty$, give the normal mode solutions
%
\begin{equation}
  \left[
  \begin{array}{c}
    \tilde{v} \\ \tilde{\sigma}
  \end{array}
  \right]_{L,i}  = 
%
  \left[
  \begin{array}{c} 
    c \\ \kappa 
  \end{array}
  \right]
%
  r^{i}a_{L,0}\qquad \hbox{ for } i\le 0 
  \label{eq:ulsol}
\end{equation}
and
\begin{equation}
  \left[
  \begin{array}{c}
    \tilde{v} \\ \tilde{\sigma}
  \end{array}
  \right]_{R,i}  = 
%
  \left[
  \begin{array}{c} 
    -c \\ \kappa
  \end{array}
  \right]
%
  r^{-i}b_{R,0} \qquad \hbox{ for } i\ge 0,
  \label{eq:ursol}
\end{equation}
where $r=\frac{A-1+\lambda}{\lambda}$ and $\lambda = \frac{c\dt}{\dx}$. The CFL condition for the upwind
discretization of the fluid domains is $\lambda <1$. The solutions (\ref{eq:ulsol}) and (\ref{eq:ursol}) 
are bounded because $|r| > 1$. To see that this inequality holds, rewrite $|r|^2>1$ in terms of the polar 
variables $R$ and $\theta$, where $A = R e^{i\theta}$. By simple algebraic 
manipulations, $|r|^2 > 1$ can be rewritten as
$$
  (R-1)^2 + 2\lambda(R-1) + 2R(1-\lambda)(1-\cos\theta) > 0,
$$
which is true since $R>1$ and $\lambda<1$.

Three equations for the undetermined constants $a_{L,0}$ and $b_{R,0}$ and the unknown $\tilde{v}_M$ are 
obtained by application of the interface conditions (\ref{eq:vLeftFO})-(\ref{eq:stressRightFO}) and the 
rigid body integrator (\ref{eq:BE}). This leads to the linear system of equations
\begin{equation}
  \left[
  \begin{array}{ccc}
    \displaystyle{1-\frac{1}{2r}+\frac{\alpha c}{2\kappa r}} & 0 & \displaystyle{-\frac{1}{2c}-\frac{\alpha}{2\kappa}} \medskip \\
    0 & \displaystyle{1-\frac{1}{2r}+\frac{\alpha c}{2\kappa r}} & \displaystyle{\frac{1}{2c}+\frac{\alpha}{2\kappa}} \medskip \\
    \displaystyle{\frac{A\xi}{r}\left(\kappa-\alpha c\right)} & \displaystyle{-\frac{A\xi}{r}\left(\kappa-\alpha c\right)} & \displaystyle{A-1+2\xi\alpha A}
  \end{array}
  \right]
  %
  \left[
  \begin{array}{c}
    a_{L,0} \medskip \\ b_{R,0} \medskip \\ \tilde{\vRB}
  \end{array}
  \right] = 0
  \label{eq:eig}
\end{equation}
%
where $\xi=\frac{\dt}{\mass}$. The system (\ref{eq:eig}) is an eigenvalue problem for $A$, in
the sense that if there is an $A$ such that the determinant of the system is zero, then there exists 
a non-trivial solution of the form (\ref{eq:normalmode}). If, furthermore, $|A|>1$, then the 
solution (\ref{eq:normalmode}) grows in time. 
%The determinant condition says that nontrivial solutions exist when the determinant
%equals zero which can be manipulated to yield a polynomial in $A$.
\begin{theorem}
The numerical scheme using the interior discretizations (\ref{eq:discreteInterior_fo}), 
interface conditions (\ref{eq:vLeftFO})-(\ref{eq:stressRightFO}), rigid body integrator (\ref{eq:BE}) 
and projections (\ref{eq:genStressLeft})-(\ref{eq:genStressRight}) with $\alpha=\rho c$ has no 
eigenvalues $A$ with $|A|>1$ for $\lambda \le 1$ and $\mass > 0$.
  \label{thm:projectedFO}
\end{theorem}
%
\begin{proof}
For $\alpha=\rho c$ the eigenvalue problem (\ref{eq:eig}) reduces to 
%
\begin{equation}
  \left[
  \begin{array}{ccc}
    \displaystyle{1} & 0 & \displaystyle{-\frac{1}{c}} \medskip \\
    0 & \displaystyle{1} & \displaystyle{\frac{1}{c}} \medskip \\
    0 & 0 & \displaystyle{A-1+2\xi\rho c A}
  \end{array}
  \right]
  %
  \left[
  \begin{array}{c}
    a_{L,0} \medskip \\ b_{R,0} \medskip \\ \tilde{\vRB}
  \end{array}
  \right] = 0.
\end{equation}%
The determinant is zero when $A= \frac{1}{1+2\xi\rho c}$. By assumption, $\xi=\frac{\dt}{\mass} > 0$, $\rho>0$, and $c>0$ and so $|A| < 1$. Recall that the interior discretizations (\ref{eq:discreteInterior_fo}) are stable for $\lambda \le 1$ and this completes the proof.
\end{proof}

\begin{theorem}
The numerical scheme using the interior discretizations (\ref{eq:discreteInterior_fo}), interface 
conditions (\ref{eq:vLeftFO})-(\ref{eq:stressRightFO}), rigid body integrator (\ref{eq:BE}) and 
projections (\ref{eq:genStressLeft})-(\ref{eq:genStressRight}) with $\alpha=0$ has no eigenvalues $A$ with
$|A|>1$ when 
\begin{equation}
\Delta t < M(4-\lambda)/(\rho c\lambda)
\label{eq:trestr}
\end{equation}
for $\lambda \leq 1$. Conversely, if 
$\Delta t > M(4-\lambda)/(\rho c\lambda)$, then there are eigenvalues with $|A|>1$ for $\lambda \leq 1$.
\label{thm:traditionalFO}
\end{theorem}
%
\begin{proof}
For $\alpha=0$, the eigenvalue problem (\ref{eq:eig}) reduces to
%
\begin{equation}
  \left[
  \begin{array}{ccc}
    \displaystyle{1-\frac{1}{2r}} & 0 & \displaystyle{-\frac{1}{2c}} \medskip \\
    0 & \displaystyle{1-\frac{1}{2r}} & \displaystyle{\frac{1}{2c}} \medskip \\
    \displaystyle{\frac{A\xi}{r}\kappa} & \displaystyle{-\frac{A\xi}{r}\kappa} & \displaystyle{A-1}
  \end{array}
  \right]
  %
  \left[
  \begin{array}{c}
    a_{L,0} \medskip \\ b_{R,0} \medskip \\ \tilde{\vRB}
  \end{array}
  \right] = 0.
\end{equation}
%
The zero determinant condition is solved to give three roots $A_1=1-\frac{\lambda}{2}$ and 
\begin{equation}
A_{2,3}=1-\frac{\lambda}{4}-\frac{\rho c \xi \lambda}{2} \pm 
                \sqrt{ \left(1-\frac{\lambda}{4}-\frac{\rho c \xi \lambda}{2}\right)^2 -1 +\frac{\lambda}{2} }
\label{eq:roots23}
\end{equation}
Clearly, $|A_1|<1$ for $\lambda \leq 1$. In the case
$$
\left(1-\frac{\lambda}{4}-\frac{\rho c \xi \lambda}{2}\right)^2 -1 +\frac{\lambda}{2} < 0,
$$
$A_2$ and $A_3$ are complex conjugate, and 
$$
 |A_2|^2=|A_3|^2 = (1-\frac{\lambda}{4}-\frac{\rho c \xi \lambda}{2})^2 + 
(1-\frac{\lambda}{4}-\frac{\rho c \xi \lambda}{2})^2 + 1 - \frac{\lambda}{2} = 1 -\frac{\lambda}{2} < 1
$$
When $A_2$ and $A_3$ are real, rewriting (\ref{eq:roots23}) as
$$
A_{2,3}=1-(\frac{\lambda}{4}+\frac{\rho c \xi \lambda}{2}) \pm 
                \sqrt{ \left(\frac{\lambda}{4}+\frac{\rho c \xi \lambda}{2}\right)^2 -\rho c\xi\lambda}
$$
shows directly that both roots are are always $ <1$, hence $|A|<1$ 
if and only if
$$
 -1 < 1-(\frac{\lambda}{4}+\frac{\rho c \xi \lambda}{2}) - 
             \sqrt{ \left(\frac{\lambda}{4}+\frac{\rho c \xi \lambda}{2}\right)^2 -\rho c\xi\lambda}
$$
which is equivalent to
\begin{equation}
 \sqrt{ \left(\frac{\lambda}{4}+\frac{\rho c \xi \lambda}{2}\right)^2 -\rho c\xi\lambda} 
            < 2-(\frac{\lambda}{4}+\frac{\rho c \xi \lambda}{2}).
\label{eq:negcond}
\end{equation}
The necessary condition that the right hand side is positive is equivalent to
\begin{equation}
  \rho c\xi\lambda < 4 - \frac{\lambda}{2}.
\label{eq:poscond}
\end{equation}
Assume (\ref{eq:poscond}) holds and square both sides of (\ref{eq:negcond}) to obtain
\begin{equation}
  \rho c\xi\lambda < 4 - \lambda.
\label{eq:finalcond}
\end{equation}
Hence, $|A|<1$ exactly when (\ref{eq:finalcond}) holds. The proof is completed by observing that
(\ref{eq:finalcond}) is equivalent to (\ref{eq:trestr}).
\end{proof}
Theorem~\ref{thm:traditionalFO} means that an explicit ODE type of time step restriction exists, even though
(\ref{eq:RBMotion}) is integrated by an unconditionally stable ODE integrator. In the case of light 
bodies, i.e., bodies with small $M$, this time step restriction is very severe. 
Another way to state the result is that for any fixed grid resolution, there exists some 
sufficiently small mass that the scheme will give a solution that grows exponentially in time. 
In fact, it is easy to see that for $\alpha=0$  and 
fixed $\dt$, the limit of small mass yields $r\to1-\frac{\lambda}{4}-\frac{\rho c\lambda\dt}{\mass}$ and 
therefore $\lim_{\mass\to0}|A|=\infty$. 
\par
Theorem~\ref{thm:projectedFO} shows that the time step restriction (\ref{eq:trestr}) is easy to avoid 
by switching to the interface conditions with $\alpha=\rho c$.
Note however, that the method is stable in the sense of PDE stability, also when $\alpha=0$, since 
the eigenvalues will eventually be smaller than one when $\Delta x$ and $\Delta t \rightarrow$ 0, 
for fixed $\lambda$. 
\par
The structure of the eigenvalue problem in the proof of Theorem~\ref{thm:projectedFO} shows why the
choice $\alpha=\rho c$ is in some sense optimal. Because $\kappa-\rho c^2 = 0$ the evolution of the rigid body 
equations is decoupled from the evolution of two fluid domains and stability for any nonnegative rigid body mass 
is obtained. This is the primary implication of Theorem~\ref{thm:projectedFO}. On the other hand, for $\alpha=0$,
the eigenvalue problem (\ref{eq:eig}) represents a coupled system and the question of stability is summarized in
Theorem~\ref{thm:traditionalFO}. 
\par
For choices of $\alpha$ other than zero or $\rho c$, the stability of the numerical scheme 
varies somewhat. The determinant condition can be used to produce an expression for $A$, but it is somewhat
difficult to interpret. We provide no further discussion about other choices of the parameter $\alpha$.


%It is particularly informative to study the limiting behavior of the roots of the determinant condition for very large and very small masses. Looking at the behavior as a function of $\alpha$ indicates why $\alpha=\rho c$ is in some sense the "best" choice. For the very large mass case,
%%
%\begin{align}
%  \mass\to\infty \Rightarrow\left\{
%      \begin{array}{ccc}
%        r_1 & \to & 1-\frac{\lambda}{2}-\frac{\alpha c\lambda}{2\kappa} \medskip\\
%        r_2 & \to & 1^{-} \medskip \\
%        r_3 & \to & 1-\frac{\lambda}{2}-\frac{\alpha c\lambda}{2\kappa}.
%      \end{array}
%  \right.
%\end{align}
%%
%Here the notation $1^{-}$ indicates that the approach is from the bottom. For the very small mass case,
%\begin{align}
%  \mass\to 0 \Rightarrow\left\{
%      \begin{array}{ccc}
%        r_1 & \to & 1-\frac{\lambda}{2}-\frac{\alpha c\lambda}{2\kappa} \medskip\\
%        r_2 & \to & \frac{1}{4}\left(2-\lambda-\frac{\kappa\lambda}{\alpha c}+\frac{\left|\kappa\lambda-2\alpha c+\alpha\lambda c\right|}{\alpha c}\right) \medskip \\
%        r_3 & \to & \frac{1}{4}\left(2-\lambda-\frac{\kappa\lambda}{\alpha c}-\frac{\left|\kappa\lambda-2\alpha c+\alpha\lambda c\right|}{\alpha c}\right)
%      \end{array}
%  \right.
%\end{align}
%The points I would make here are the following. Firstly, for $\alpha=\rho c$, all $\alpha$ dependence for the large and small mass cases goes away and we get 
%\begin{align}
%  \mass\to\infty \Rightarrow\left\{
%      \begin{array}{ccc}
%        r_1 & \to & 1-\lambda \medskip\\
%        r_2 & \to & 1^{-} \medskip \\
%        r_3 & \to & 1-\lambda
%      \end{array}
%  \right., \qquad
%  %
%  \mass\to 0 \Rightarrow\left\{
%      \begin{array}{ccc}
%        r_1 & \to & 1-\lambda \medskip\\
%        r_2 & \to & 1-\lambda \medskip \\
%        r_3 & \to & 0.
%      \end{array}
%  \right.
%\end{align}
%This has the added advantage that all roots are positive in the limit and so the normal mode for the $\vRB$ is strictly decaying. Secondly, for $\alpha\ne\rho c$ and $\alpha\ne 0$, some dependence on $\alpha$ is acquired which puts restrictions on the choice of $\alpha$ if stability for the limiting mass cases is desired (I think $0 \le \alpha \le \rho c$). Thirdly, for $\alpha=0$ the small mass limit is problematic with $r_3$ going like $-\frac{\dt\kappa\lambda}{c\mass}$. Thus, for $\alpha=0$  and fixed $\dt$, $\lim_{\mass\to0}r_3=-\infty$.

%What this is all saying in words is that if you use the traditional application of interface conditions with a partitioned approach, you can pick up an ODE-like stability constraint even if you integrate the solid body motion in a stable manner. On the flip side if you use the projection with impedance weighting, this stability constraint can be avoided. Furthermore, if one looks at the structure of the eigenvalue problem defining stability, it is rather easy to see why the optimal weighting for the pressure projection is the impedance $z=\rho c$. Note that because the stability of the rigid body ODE is separated from the stability of the fluids, any stable time stepper can be used for the solid and still obtain stability for the projection technique. In particular, a forward Euler integrator with a fixed and known number of sub-cycles can be used. For this kind of sub-cyling algorithm, the pressure projection ensures stability when the small time steps (with $\dt\approx\frac{\mass}{\rho c}$) are taken for the ODE only. Without the projection, the entire system must be stepped at the smaller time step because of the dynamics of the solids and fluids are linked by the partitioning. Finally I note that the decoupling of the rigid body equations from the fluid equations also occurs for $\kappaL\ne\kappaR$ of $\rhoL\ne\rhoR$.

%One interesting limit to investigate is to look at the determinant condition for filed CFL $\lambda = \frac{c\dt}{\dx}$ while $\dt\to\infty$. The "bad" eigenvalue for this case goes like
%\[
%  1-\frac{\lambda}{2}-\frac{\lambda}{4\alpha c}(1+\kappa).
%\]
%This is telling us that for any mass body and sufficiently coarse mesh, the traditional coupling strategy with $\alpha=0$ is unstable. 

